Text encoders bottleneck compositionality in contrastive vision-language models

Performant vision-language (VL) models like CLIP represent captions using a single vector. How much information about language is lost in this bottleneck? We first curate CompPrompts, a set of increasingly compositional image captions that VL models should be able to capture (e.g., single object, to object+property, to multiple interacting objects). Then, we train text-only recovery probes that aim to reconstruct captions from single-vector text representations produced by several VL models. This approach does not require images, allowing us to test on a broader range of scenes compared to prior work. We find that: 1) CLIP's text encoder falls short on more compositional inputs, including object relationships, attribute-object association, counting, and negations; 2) some text encoders work significantly better than others; and 3) text-only recovery performance predicts multi-modal matching performance on ControlledImCaps: a new evaluation benchmark we collect and release consisting of fine-grained compositional images and captions. Specifically, our results suggest text-only recoverability is a necessary (but not sufficient) condition for modeling compositional factors in contrastive VL models. We release our datasets and code.

==> autotable.tex <==
%Please add the following packages if necessary:
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
%\begin{table}[!htp]\centering
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{  
\begin{tabular}{lrrrrrrrrrrrrrrrr}\toprule
CLIP\\ViT-B/32\\T5-large &\textbf{0 attributes} &\multicolumn{4}{c}{\textbf{1 attribute}} &\multicolumn{10}{c}{\textbf{2 attributes}} \\\cmidrule{1-16}
& &1 adjective &1 spatial &1 SOV &1 DOV &2 adjectives &1 adj + 1 spatial &1 adj + 1 SOV &1 adj + 1 DOV &1 spatial + 1 SOV &1 spatial + 1 DOV &2 spatial &1 temporal + 1 SOV &1 temporal + 1 DOV &2 verbs \\\midrule
\textbf{1 unique object} &a cat &an orange cat &a cat on the left &a cat yawning &- &an orange and spotted cat &an orange cat on the left &an orange cat yawning & &a cat on the left yawning & & &a cat before yawning & & \\
\textbf{} &25.3 &72.4 &67.6 &55 & &11.2 &49.2 &51 & &7.2 & & &39.6 & & \\
\textbf{2 unique objects} &a cat and a dog &an orange cat and a dog / a cat and a brown dog &a cat to the left of a dog &a cat yawning and a dog &a cat chasing a dog &an orange cat and a brown dog &an orange cat to the left of a dog &a cat yawning and a brown dog &a cat chasing a brown dog / an orange cat chasing a dog &a cat yawning to the left of a dog &a cat chasing a dog on the left &a cat on the right and a dog on the left &a cat before yawning and a dog &a cat before chasing a dog &a cat yawning and a dog stretching \\
\textbf{} &46.6 &27 &14.6 &0.8 &29 &16.2 &6.7 &0.4 &11.8 &8.3 &5 &1.8 &0.6 &8 &1.4 \\
\textbf{1 unique object + multiples} &2 cats &2 orange cats &X cats on the left &X cats yawning &- & & & & & & & & & & \\
\textbf{} &0.3 &4.4 &2.8 &2.8 & & & & & & & & & & & \\
\textbf{2 unique objects + multiples} &2 cats and 4 dogs &- &X cats to the left of Y dogs &- &X cats chasing Y dogs & & & & & & & & & & \\
\textbf{} &0 & &0 & &0 & & & & & & & & & & \\
\textbf{1 unique object + negation} &- &a cat that is not orange &a cat that is not on the left &a cat that is not yawning &- & & & & & & & & & & \\
\textbf{} & &13 &0.2 &9.4 & & & & & & & & & & & \\
\textbf{2 unique objects + negation} &- &- &a cat that is not to the left of a dog &- &a cat that is not chasing a dog & & & & & & & & & & \\
\textbf{} & & &0.2 & &0.4 & & & & & & & & & & \\
\bottomrule
\end{tabular}}
\end{table*}


==> tables/clip_em.tex <==
% Auto-generated, please don't judge
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{  

\begin{tabular}{|l|l|llll|llllllllll|}
\hline
                & \multicolumn{1}{c|}{\textbf{0 attributes}}                                       & \multicolumn{4}{c|}{\textbf{1 attribute}}                                                                                                                                                                                                                                                                                                                                                                                                            & \multicolumn{10}{c|}{\textbf{2 attributes}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                        \\ \hline
                                                                                                        &                                                                      & \multicolumn{1}{c|}{1 adj.}                                                                                                          & \multicolumn{1}{c|}{1 spatial}                                                                                      & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}1 1-obj\\ verb\end{tabular}}                         & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}1 2-obj\\ verb\end{tabular}}             & \multicolumn{1}{c|}{2 adj}                                                                              & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}1 adj +\\ 1 spatial\end{tabular}}                               & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}1 adj + \\ 1 1-obj\\ verb\end{tabular}}                      & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}1 adj + \\ 1 2-obj\\ verb\end{tabular}}                                                      & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}1 spatial\\ + 1 1-obj\\ verb\end{tabular}}                         & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}1 spatial\\ + 1 2-obj\\ verb\end{tabular}}                   & \multicolumn{1}{c|}{2 spatial}                                                                                       & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}1 temp \\ + 1 1-obj\\ verb\end{tabular}}                     & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}1 temp \\ + 1 2-obj\\ verb\end{tabular}}                 & \multicolumn{1}{c|}{2 verbs}                                                               \\ \hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}1 unique \\ object\end{tabular}}}               & \textit{a cat}                                                       & \multicolumn{1}{l|}{\textit{\begin{tabular}[c]{@{}l@{}}an orange \\cat\end{tabular}}}                                                                                                 & \multicolumn{1}{l|}{\textit{\begin{tabular}[c]{@{}l@{}}a cat on\\ the left\end{tabular}}}                           & \multicolumn{1}{l|}{\textit{\begin{tabular}[c]{@{}l@{}}a cat\\ yawning\end{tabular}}}               & \textit{-}                                                                              & \multicolumn{1}{l|}{\textit{\begin{tabular}[c]{@{}l@{}}an orange\\ and\\ spotted cat\end{tabular}}}     & \multicolumn{1}{l|}{\textit{\begin{tabular}[c]{@{}l@{}}an orange\\ cat on\\ the left\end{tabular}}}            & \multicolumn{1}{l|}{\textit{\begin{tabular}[c]{@{}l@{}}an orange\\ cat\\ yawning\end{tabular}}}             & \multicolumn{1}{l|}{}                                                                                                                       & \multicolumn{1}{l|}{\textit{\begin{tabular}[c]{@{}l@{}}a cat on\\ the left\\ yawning\end{tabular}}}               & \multicolumn{1}{l|}{}                                                                                       & \multicolumn{1}{l|}{}                                                                                                & \multicolumn{1}{l|}{\textit{\begin{tabular}[c]{@{}l@{}}a cat \\ before\\ yawning\end{tabular}}}             & \multicolumn{1}{l|}{}                                                                                   &                                                                                            \\ 
                                                                                                        & \multicolumn{1}{r|}{25.3}                                            & \multicolumn{1}{r|}{72.4}                                                                                                      & \multicolumn{1}{r|}{67.6}                                                                                           & \multicolumn{1}{r|}{55}                                                                             &                                                                                         & \multicolumn{1}{r|}{11.2}                                                                               & \multicolumn{1}{r|}{49.2}                                                                                      & \multicolumn{1}{r|}{51}                                                                                     & \multicolumn{1}{l|}{}                                                                                                                       & \multicolumn{1}{r|}{7.2}                                                                                          & \multicolumn{1}{l|}{}                                                                                       & \multicolumn{1}{l|}{}                                                                                                & \multicolumn{1}{r|}{39.6}                                                                                   & \multicolumn{1}{l|}{}                                                                                   &                                                                                            \\ \hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}2 unique \\ objects\end{tabular}}}              & \textit{\begin{tabular}[c]{@{}l@{}}a cat and\\ a dog\end{tabular}}   & \multicolumn{1}{l|}{\textit{\begin{tabular}[c]{@{}l@{}}an orange\\ cat and a\\ dog / a cat\\ and a \\ brown dog\end{tabular}}} & \multicolumn{1}{l|}{\textit{\begin{tabular}[c]{@{}l@{}}a cat to\\ the left\\ of a dog\end{tabular}}}                & \multicolumn{1}{l|}{\textit{\begin{tabular}[c]{@{}l@{}}a cat\\ yawning\\ and a\\ dog\end{tabular}}} & \textit{\begin{tabular}[c]{@{}l@{}}a cat\\ chasing\\ a dog\end{tabular}}                & \multicolumn{1}{l|}{\textit{\begin{tabular}[c]{@{}l@{}}an orange\\ cat and a\\ brown dog\end{tabular}}} & \multicolumn{1}{l|}{\textit{\begin{tabular}[c]{@{}l@{}}an orange\\ cat to the\\ left of a\\ dog\end{tabular}}} & \multicolumn{1}{l|}{\textit{\begin{tabular}[c]{@{}l@{}}a cat \\ yawning\\ and a \\ brown dog\end{tabular}}} & \multicolumn{1}{l|}{\textit{\begin{tabular}[c]{@{}l@{}}a cat\\ chasing\\ a brown\\ dog / an \\ orange cat\\ chasing \\ a dog\end{tabular}}} & \multicolumn{1}{l|}{\textit{\begin{tabular}[c]{@{}l@{}}a cat\\ yawning\\ to the\\ left of a \\ dog\end{tabular}}} & \multicolumn{1}{l|}{\textit{\begin{tabular}[c]{@{}l@{}}a cat\\ chasing a\\ dog on the\\ left\end{tabular}}} & \multicolumn{1}{l|}{\textit{\begin{tabular}[c]{@{}l@{}}a cat on\\ the right\\ and a dog\\ on the left\end{tabular}}} & \multicolumn{1}{l|}{\textit{\begin{tabular}[c]{@{}l@{}}a cat \\ before\\ yawning\\ and a dog\end{tabular}}} & \multicolumn{1}{l|}{\textit{\begin{tabular}[c]{@{}l@{}}a cat\\ before\\ chasing \\ a dog\end{tabular}}} & \textit{\begin{tabular}[c]{@{}l@{}}a cat \\ yawning\\ and a dog\\ stretching\end{tabular}} \\
                                                                                                        & \multicolumn{1}{r|}{46.6}                                            & \multicolumn{1}{r|}{27}                                                                                                        & \multicolumn{1}{r|}{14.6}                                                                                           & \multicolumn{1}{r|}{0.8}                                                                            & \multicolumn{1}{r|}{29}                                                                 & \multicolumn{1}{r|}{16.2}                                                                               & \multicolumn{1}{r|}{6.7}                                                                                       & \multicolumn{1}{r|}{0.4}                                                                                    & \multicolumn{1}{r|}{11.8}                                                                                                                   & \multicolumn{1}{r|}{8.3}                                                                                          & \multicolumn{1}{r|}{5}                                                                                      & \multicolumn{1}{r|}{1.8}                                                                                             & \multicolumn{1}{r|}{0.6}                                                                                    & \multicolumn{1}{r|}{8}                                                                                  & \multicolumn{1}{r|}{1.4}                                                                   \\ \hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}1 unique\\ object +\\ multiples\end{tabular}}}  & \textit{2 cats}                                                      & \multicolumn{1}{l|}{\textit{\begin{tabular}[c]{@{}l@{}}2 orange\\ cats\end{tabular}}}                                          & \multicolumn{1}{l|}{\textit{\begin{tabular}[c]{@{}l@{}}X cats on\\ the left\end{tabular}}}                          & \multicolumn{1}{l|}{\textit{\begin{tabular}[c]{@{}l@{}}X cats\\ yawning\end{tabular}}}              & \textit{-}                                                                              & \multicolumn{1}{l|}{}                                                                                   & \multicolumn{1}{l|}{}                                                                                          & \multicolumn{1}{l|}{}                                                                                       & \multicolumn{1}{l|}{}                                                                                                                       & \multicolumn{1}{l|}{}                                                                                             & \multicolumn{1}{l|}{}                                                                                       & \multicolumn{1}{l|}{}                                                                                                & \multicolumn{1}{l|}{}                                                                                       & \multicolumn{1}{l|}{}                                                                                   &                                                                                            \\ 
                                                                                                        & \multicolumn{1}{r|}{0.3}                                             & \multicolumn{1}{r|}{4.4}                                                                                                       & \multicolumn{1}{r|}{2.8}                                                                                            & \multicolumn{1}{r|}{2.8}                                                                            &                                                                                         & \multicolumn{1}{l|}{}                                                                                   & \multicolumn{1}{l|}{}                                                                                          & \multicolumn{1}{l|}{}                                                                                       & \multicolumn{1}{l|}{}                                                                                                                       & \multicolumn{1}{l|}{}                                                                                             & \multicolumn{1}{l|}{}                                                                                       & \multicolumn{1}{l|}{}                                                                                                & \multicolumn{1}{l|}{}                                                                                       & \multicolumn{1}{l|}{}                                                                                   &                                                                                            \\ \hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}2 unique\\ objects +\\ multiples\end{tabular}}} & \textit{\begin{tabular}[c]{@{}l@{}}2 cats and\\ 4 dogs\end{tabular}} & \multicolumn{1}{l|}{\textit{-}}                                                                                                & \multicolumn{1}{l|}{\textit{\begin{tabular}[c]{@{}l@{}}X cats to\\ the left\\ of Y dogs\end{tabular}}}              & \multicolumn{1}{l|}{\textit{-}}                                                                     & \textit{\begin{tabular}[c]{@{}l@{}}X cats\\ chasing\\ Y dogs\end{tabular}}              & \multicolumn{1}{l|}{}                                                                                   & \multicolumn{1}{l|}{}                                                                                          & \multicolumn{1}{l|}{}                                                                                       & \multicolumn{1}{l|}{}                                                                                                                       & \multicolumn{1}{l|}{}                                                                                             & \multicolumn{1}{l|}{}                                                                                       & \multicolumn{1}{l|}{}                                                                                                & \multicolumn{1}{l|}{}                                                                                       & \multicolumn{1}{l|}{}                                                                                   &                                                                                            \\ 
                                                                                                        & \multicolumn{1}{r|}{0}                                               & \multicolumn{1}{l|}{}                                                                                                          & \multicolumn{1}{r|}{0}                                                                                              & \multicolumn{1}{l|}{}                                                                               & \multicolumn{1}{r|}{0}                                                                  & \multicolumn{1}{l|}{}                                                                                   & \multicolumn{1}{l|}{}                                                                                          & \multicolumn{1}{l|}{}                                                                                       & \multicolumn{1}{l|}{}                                                                                                                       & \multicolumn{1}{l|}{}                                                                                             & \multicolumn{1}{l|}{}                                                                                       & \multicolumn{1}{l|}{}                                                                                                & \multicolumn{1}{l|}{}                                                                                       & \multicolumn{1}{l|}{}                                                                                   &                                                                                            \\ \hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}1 unique\\ object +\\ negation\end{tabular}}}   & \textit{-}                                                           & \multicolumn{1}{l|}{\textit{\begin{tabular}[c]{@{}l@{}}a cat that\\ is not\\ orange\end{tabular}}}                             & \multicolumn{1}{l|}{\textit{\begin{tabular}[c]{@{}l@{}}a cat that\\ is not on\\ the left\end{tabular}}}             & \multicolumn{1}{l|}{\textit{\begin{tabular}[c]{@{}l@{}}a cat that\\ is not\\ yawning\end{tabular}}} & \textit{-}                                                                              & \multicolumn{1}{l|}{}                                                                                   & \multicolumn{1}{l|}{}                                                                                          & \multicolumn{1}{l|}{}                                                                                       & \multicolumn{1}{l|}{}                                                                                                                       & \multicolumn{1}{l|}{}                                                                                             & \multicolumn{1}{l|}{}                                                                                       & \multicolumn{1}{l|}{}                                                                                                & \multicolumn{1}{l|}{}                                                                                       & \multicolumn{1}{l|}{}                                                                                   &                                                                                            \\ 
                                                                                                        &                                                                      & \multicolumn{1}{r|}{13}                                                                                                        & \multicolumn{1}{r|}{0.2}                                                                                            & \multicolumn{1}{r|}{9.4}                                                                            &                                                                                         & \multicolumn{1}{l|}{}                                                                                   & \multicolumn{1}{l|}{}                                                                                          & \multicolumn{1}{l|}{}                                                                                       & \multicolumn{1}{l|}{}                                                                                                                       & \multicolumn{1}{l|}{}                                                                                             & \multicolumn{1}{l|}{}                                                                                       & \multicolumn{1}{l|}{}                                                                                                & \multicolumn{1}{l|}{}                                                                                       & \multicolumn{1}{l|}{}                                                                                   &                                                                                            \\ \hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}2 unique\\ objects +\\ negation\end{tabular}}}  & \textit{-}                                                           & \multicolumn{1}{l|}{\textit{-}}                                                                                                & \multicolumn{1}{l|}{\textit{\begin{tabular}[c]{@{}l@{}}a cat that\\ is not to\\ the left \\ of a dog\end{tabular}}} & \multicolumn{1}{l|}{\textit{-}}                                                                     & \textit{\begin{tabular}[c]{@{}l@{}}a cat that\\ is not\\ chasing \\ a dog\end{tabular}} & \multicolumn{1}{l|}{}                                                                                   & \multicolumn{1}{l|}{}                                                                                          & \multicolumn{1}{l|}{}                                                                                       & \multicolumn{1}{l|}{}                                                                                                                       & \multicolumn{1}{l|}{}                                                                                             & \multicolumn{1}{l|}{}                                                                                       & \multicolumn{1}{l|}{}                                                                                                & \multicolumn{1}{l|}{}                                                                                       & \multicolumn{1}{l|}{}                                                                                   &                                                                                            \\ 
                                                                                                        &                                                                      & \multicolumn{1}{l|}{}                                                                                                          & \multicolumn{1}{r|}{0.2}                                                                                            & \multicolumn{1}{l|}{}                                                                               & \multicolumn{1}{r|}{0.4}                                                                & \multicolumn{1}{l|}{}                                                                                   & \multicolumn{1}{l|}{}                                                                                          & \multicolumn{1}{l|}{}                                                                                       & \multicolumn{1}{l|}{}                                                                                                                       & \multicolumn{1}{l|}{}                                                                                             & \multicolumn{1}{l|}{}                                                                                       & \multicolumn{1}{l|}{}                                                                                                & \multicolumn{1}{l|}{}                                                                                       & \multicolumn{1}{l|}{}                                                                                   &                                                                                            \\ \hline
\end{tabular}
}\end{table*}

==> tables/clip_em_2.tex <==
\begin{table*}[ht]
\resizebox{\textwidth}{!}{ 
\begin{tabular}{lcc@{}c@{}c@{}cc@{}c@{}c@{}c@{}c@{}c@{}c@{ }c@{}c@{}c@{}c}
 &\textbf{0 attributes} &\multicolumn{4}{c}{\textbf{1 attribute}} &\multicolumn{10}{c}{\textbf{2 attributes}} \\\cmidrule(lr){3-6}\cmidrule(lr){7-16}
& &1 adj. &1 spatial &\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}1 1-obj \\ verb\end{tabular}} &\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}1 2-obj \\ verb\end{tabular}} &2 adj. &\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}1 adj + \\ 1 spatial\end{tabular}} &\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}1 adj + \\ 1 1-obj \\ verb\end{tabular}} &\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}1 adj + \\ 1 2-obj \\ verb\end{tabular}} &\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}1 spatial \\ + 1 1-obj \\ verb\end{tabular}} &\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}} 1 spatial \\ + 1 2-obj \\verb\end{tabular}} &2 spatial &\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}1 temp. + \\ 1 1-obj \\ verb\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}1 temp. + \\ 1 2-obj \\ verb\end{tabular}} &2 verbs \\\midrule
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}1 unique \\ object\end{tabular}}} &\multicolumn{1}{l}{\textit{a cat}}& \textit{\begin{tabular}[l]{l}an orange\\ cat\end{tabular}} &\textit{\begin{tabular}[l]{l}a cat on\\ the left\end{tabular}} &\textit{\begin{tabular}[l]{l}a cat \\ yawning\end{tabular}} & - & \textit{\begin{tabular}[l]{l}an orange\\ and spotted\\ cat\end{tabular}} &\textit{\begin{tabular}[l]{l}an orange\\ cat on \\ the left\end{tabular}}& \textit{\begin{tabular}[l]{l}an orange\\ cat \\ yawning\end{tabular}} & - &\textit{\begin{tabular}[l]{l}a cat on \\ the left \\yawning\end{tabular}} & - & - &\textit{\begin{tabular}[l]{l}a cat\\ before \\ yawning\end{tabular}} & - & - \\
\textbf{} &\multicolumn{1}{r}{33.0} &\multicolumn{1}{r}{81.8} &\multicolumn{1}{r}{53.2} &\multicolumn{1}{r}{71.6} & &\multicolumn{1}{r}{23.2} &\multicolumn{1}{r}{43.8} &\multicolumn{1}{r}{62.6} & &\multicolumn{1}{r}{6.2} & & &\multicolumn{1}{r}{58.6} & & \\\cmidrule{1-16}
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}2 unique \\ objects\end{tabular}}} &\textit{\begin{tabular}[l]{l}a cat and\\ a dog\end{tabular}} & \textit{\begin{tabular}[l]{l}an orange\\ cat and a \\ dog / a cat \\ and a \\ brown dog\end{tabular}} & \textit{\begin{tabular}[l]{l}a cat to\\ the left \\ of a dog\end{tabular}} &\textit{\begin{tabular}[l]{l}a cat \\ yawning \\ and a \\dog\end{tabular}} & \textit{\begin{tabular}[l]{l}a cat\\ chasing \\ a dog\end{tabular}} & \textit{\begin{tabular}[l]{l}an orange\\ cat and a \\ brown dog\end{tabular}} &\textit{\begin{tabular}[l]{l}an orange \\cat to the \\ left of a \\ dog\end{tabular}} & \textit{\begin{tabular}[l]{l}a cat \\yawning \\ and a \\ brown dog\end{tabular}}  &\textit{\begin{tabular}[l]{l}a cat \\chasing \\a brown \\dog / an \\orange cat \\chasing \\a dog\end{tabular}}&\textit{\begin{tabular}[l]{l}a cat \\yawning \\to the \\left of a \\dog\end{tabular}} & \textit{\begin{tabular}[l]{l}a cat \\chasing a \\dog on the \\left\end{tabular}} &\textit{\begin{tabular}[l]{l}a cat on \\the right \\and a dog \\on the left\end{tabular}} &\textit{\begin{tabular}[l]{l}a cat \\before \\yawning \\and a dog\end{tabular}} &\textit{\begin{tabular}[l]{l}a cat \\before \\chasing \\a dog\end{tabular}} &\textit{\begin{tabular}[l]{l}a cat \\yawning \\and a dog \\stretching\end{tabular}} \\
\textbf{} &\multicolumn{1}{r}{48.4} &\multicolumn{1}{r}{30.2}&\multicolumn{1}{r}{17.8} &\multicolumn{1}{r}{5.0} &\multicolumn{1}{r}{37.2} &\multicolumn{1}{r}{23.6} &\multicolumn{1}{r}{14.0} &\multicolumn{1}{r}{1.4} &\multicolumn{1}{r}{21.0} &\multicolumn{1}{r}{16.6} &\multicolumn{1}{r}{7.8} &\multicolumn{1}{r}{0.6} &\multicolumn{1}{r}{0.2} &\multicolumn{1}{r}{21.6} &\multicolumn{1}{r}{4.8} \\
% \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}1 unique\\ object +\\multiples\end{tabular}}} &\multicolumn{1}{l}{\textit{two cats}} &\textit{\begin{tabular}[l]{l}two orange\\ cats\end{tabular}} & \textit{\begin{tabular}[l]{l}two cats on\\ the left\end{tabular}} &\textit{\begin{tabular}[l]{l}two cats\\ yawning\end{tabular}} &- & & & & & & & & & & \\
% \textbf{} &\multicolumn{1}{r}{0.3} &\multicolumn{1}{r}{15.0} &\multicolumn{1}{r}{9.6} &\multicolumn{1}{r}{9.4} & & & & & & & & & & & \\ \cmidrule{1-16}
% \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}2 unique\\ objects +\\multiples\end{tabular}}} &\textit{\begin{tabular}[c]{@{}l@{}}two cats \\and \\four dogs\end{tabular}} &- & \textit{\begin{tabular}[l]{l}two cats to\\ the left of \\four dogs\end{tabular}} &- &\textit{\begin{tabular}[l]{l}two cats \\ chasing \\four dogs\end{tabular}} & & & & & & & & & & \\
% \textbf{} &\multicolumn{1}{r}{0.0} & &\multicolumn{1}{r}{0.0} & &\multicolumn{1}{r}{0.0} & & & & & & & & & & \\ \midrule
% \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}1 unique\\ object +\\negation\end{tabular}}} &- & \textit{\begin{tabular}[l]{l}a cat that\\ is not \\orange\end{tabular}} &\textit{\begin{tabular}[l]{l}a cat that\\ is not on \\the left\end{tabular}}& \textit{\begin{tabular}[l]{l}a cat that\\ is not \\yawning\end{tabular}} &- & & & & & & & & & & \\
% \textbf{} & &\multicolumn{1}{r}{13.0} &\multicolumn{1}{r}{0.2} &\multicolumn{1}{r}{9.4} & & & & & & & & & & & \\ \cmidrule{1-16}
% \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}2 unique\\ objects +\\negation\end{tabular}}} &- &- & \textit{\begin{tabular}[l]{l}a cat that \\is not to \\the left \\of a dog\end{tabular}} &- &\textit{\begin{tabular}[l]{l}a cat that \\is not \\chasing \\a dog\end{tabular}} & & & & & & & & & & \\
% \textbf{} & & &\multicolumn{1}{r}{0.2} & &\multicolumn{1}{r}{0.4} & & & & & & & & & & \\
\bottomrule
\end{tabular}}
\caption{Prompt example and exact match (\% EM) score of reconstruction from 
CLIP ViT-L/14, averaged over several hundred instances each. 
% \kw{When there is only an object, why is the performance worse than with 1obj+ 1 attribute? Also, why 1obj+1 adj+1spatial suddenly get very high performance?  }
% \jack{mention that these are averages over several 100 instances each}
}\label{tab: clip_em}
\end{table*}

==> tables/negations_multiples.tex <==
\begin{table}[t]
\resizebox{\columnwidth}{!}{ 
\begin{tabular}{lccccc}
 &\textbf{0 attributes} &\multicolumn{4}{c}{\textbf{1 attribute}}\\\cmidrule(lr){3-6}
& &1 adj. &1 spatial &\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}1 1-obj \\ verb\end{tabular}} &\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}1 2-obj \\ verb\end{tabular}} \\\midrule
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}1 unique\\ object +\\multiples\end{tabular}}} &\multicolumn{1}{l}{\textit{two cats}} &\textit{\begin{tabular}[l]{l}two orange\\ cats\end{tabular}} & \textit{\begin{tabular}[l]{l}two cats on\\ the left\end{tabular}} &\textit{\begin{tabular}[l]{l}two cats\\ yawning\end{tabular}} &- \\
\textbf{} &\multicolumn{1}{r}{3.0} &\multicolumn{1}{r}{14.8} &\multicolumn{1}{r}{10.8} &\multicolumn{1}{r}{16.8} & \\ \cmidrule{1-6}
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}2 unique\\ objects +\\multiples\end{tabular}}} &\textit{\begin{tabular}[c]{@{}l@{}}two cats \\and \\four dogs\end{tabular}} &- & \textit{\begin{tabular}[l]{l}two cats to\\ the left of \\four dogs\end{tabular}} &- &\textit{\begin{tabular}[l]{l}two cats \\ chasing \\four dogs\end{tabular}} \\
&\multicolumn{1}{r}{0.0} & &\multicolumn{1}{r}{0.0} & &\multicolumn{1}{r}{0.0} \\ \midrule
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}1 unique\\ object +\\negation\end{tabular}}} &- & \textit{\begin{tabular}[l]{l}a cat that\\ is not \\orange\end{tabular}} &\textit{\begin{tabular}[l]{l}a cat that\\ is not on \\the left\end{tabular}}& \textit{\begin{tabular}[l]{l}a cat that\\ is not \\yawning\end{tabular}} &- \\
\textbf{} & &\multicolumn{1}{r}{10.4} &\multicolumn{1}{r}{6.4} &\multicolumn{1}{r}{7.8} & \\ \cmidrule{1-6}
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}2 unique\\ objects +\\negation\end{tabular}}} &- &- & \textit{\begin{tabular}[l]{l}a cat that \\is not to \\the left \\of a dog\end{tabular}} &- &\textit{\begin{tabular}[l]{l}a cat that \\is not \\chasing \\a dog\end{tabular}} \\
\textbf{} & & &\multicolumn{1}{r}{0.4} & &\multicolumn{1}{r}{0.4} \\
\bottomrule
\end{tabular}}
\caption{CLIP ViT-L/14 EM on prompts which include multiples and negations.}\label{tab: negations_multiples}
\end{table}
